Do PAC-Learners Learn the Marginal Distribution?

The Fundamental Theorem of PAC Learning asserts that learnability of a concept class $H$ is equivalent to the $\textit{uniform convergence}$ of empirical error in $H$ to its mean, or equivalently, to the problem of $\textit{density estimation}$, learnability of the underlying marginal distribution with respect to events in $H$. This seminal equivalence relies strongly on PAC learning's `distribution-free' assumption, that the adversary may choose any marginal distribution over data. Unfortunately, the distribution-free model is known to be overly adversarial in practice, failing to predict the success of modern machine learning algorithms, but without the Fundamental Theorem our theoretical understanding of learning under distributional constraints remains highly limited. In this work, we revisit the connection between PAC learning, uniform convergence, and density estimation beyond the distribution-free setting when the adversary is restricted to choosing a marginal distribution from a known family $\mathscr{P}$. We prove that while the traditional Fundamental Theorem indeed fails, a finer-grained connection between the three fundamental notions continues to hold: 1. PAC-Learning is strictly sandwiched between two refined models of density estimation, differing only in whether the learner $\textit{knows}$ the set of well-estimated events in $H$. 2. Under reasonable assumptions on $H$ and $\mathscr{P}$, density estimation is equivalent to $\textit{uniform estimation}$, a relaxation of uniform convergence allowing non-empirical estimators. Together, our results give a clearer picture of how the Fundamental Theorem extends beyond the distribution-free setting and shed new light on the classically challenging problem of learning under arbitrary distributional assumptions.

==> old.tex <==
\section{Weak ATV-learning vs. PAC-learning}
In this section we disprove a weakened quantitative version of \Cref{conj:weak}.
\begin{theorem}\label{thm:Weak-ATV-PAC}
For all $\frac{1}{16}>\varepsilon>0$ there exists a triple $(X,\mathscr P, H)$ satisfying:
\begin{enumerate}
    \item $(X,\mathscr P, H)$ is $(\varepsilon,\delta)$-Weakly ATV-learnable in $O(\log(1/\delta))$ samples,
    \item For each $D \in \mathscr P$, $(X,D,H)$ is $\varepsilon$-covered by two functions,
    \item $(X,\mathscr P, H)$ cannot be $(1/16,1/8)$-PAC learned in any finite number of samples.
\end{enumerate} 
\end{theorem}
The intuition behind our construction is in essence that a random function restricted to random sets gives a family that is locally easy to cover (over each local set there are essentially only two functions), but globally hard to distinguish between the local sets. We will need the following lemma proving the existence of pseudorandom set systems satisfying such a property.
\begin{lemma}\label{lemma:set-system}
For every $n \in \mathbb{N}$ there exist $N=N(n,\varepsilon) \in \mathbb{N}$, a labeling $f: [N] \to \{0,1\}$, and subsets $S_1,\ldots S_{M(n,\varepsilon)} \subset [N]$ such that the following conditions hold:
\begin{enumerate}
    \item $|S_j \cap S_i| \leq 2\varepsilon^2 N$
    \item $\frac{1}{4} \leq \underset{S_i}{\mathbb{E}}[f|_{S_i}] \leq \frac{3}{4}$
    \item $\underset{i \sim [M], S \sim S_i^n}{\Pr}\left[\exists j \neq i: S \subset S_j\right] \geq 1/4$
\end{enumerate}
\end{lemma}
\begin{proof}
We appeal to the probabilistic method. Namely, we prove that for a sufficiently large choice of $N$ and $M$, we will prove that  almost every set system of $M$ $\varepsilon|N|$-size subsets satisfies these properties. With that in mind, let $S_1,\ldots,S_M \subset [N]$ be sets of size $\varepsilon|N|$ chosen independently and uniformly at random from ${[N] \choose \varepsilon|N|}$. Let $f$ be any function of support exactly $|N|/2$. We first note that as long as $N$ is sufficiently large with respect to $M$, the first two properties are immediate by Chernoff and union bounds. In particular, we have:
\begin{enumerate}
    \item $\underset{S_1,\ldots,S_M}{\Pr}[\exists i \neq j : |S_j \cap S_i| > 2\varepsilon^2 N] \leq M^2e^{-\Omega(\varepsilon^2N)}$
    \item  $\underset{S_1,\ldots,S_M}{\Pr}[\exists i : |f_{S_i} - 1/2| > 1/4] \leq Me^{-\Omega(\varepsilon N)}$
\end{enumerate}
So taking $N \geq \Omega(\log(M)/\varepsilon^2)$ we can easily make both of these probabilities as large as desired.

We now prove that the third property holds with constant probability so long as $M$ is sufficiently large with respect to $n$ and $\varepsilon^{-1}$, which is enough to prove the result. Formally, we want to show:
\[
\underset{S_1,\ldots,S_M}{\Pr}\left[ \underset{i \in M, S \sim S_i^n}{\Pr}[\exists j \neq i: S \subset S_j] > 1/4 \right] > c
\]
for any constant $c>0$. Notice that it suffices to give a good enough bound on the probability of this event over all variables, that is:
\[
\underset{S_1,\ldots,S_M,i \in M, S \sim S_i^n}{\Pr}\left[ \exists j \neq i: S \subset S_j \right] > c + (1-c)/4
\]
The trick is now to notice that by symmetry it does not matter which $i \in M$ is chosen. Therefore we have:
\begin{align*}
\underset{S_1,\ldots,S_M,i \in M, S \sim S_i^n}{\Pr}\left[ \exists j \neq i: S \subset S_j \right]&=\underset{S_1,\ldots,S_M, S \sim S_1^n}{\Pr}\left[ \exists j > 1: S \subset S_j \right] \\
&= \underset{S \sim [N]^n,S_2,\ldots,S_M}{\Pr}\left[ \exists S_j: S \subset S_j \right]
\end{align*}
where the latter equality follows from the fact that $S_2,\ldots,S_M$ are independent of $S_1$ and $S$. Notice that each $S_i$ independently has exactly a $\varepsilon^n$ probability of containing $S$. It follows that:
\[
\underset{S \sim [N]^n,S_2,\ldots,S_M}{\Pr}\left[ \exists S_j: S \subset S_j \right] = 1-(1-\varepsilon^n)^{M-1} \geq 1-e^{-\varepsilon^n(M-1)}.
\]
Therefore taking $M=\Theta(\frac{1}{\varepsilon}^n)$ we may make this probability as large as desired, which finishes the proof.
\end{proof}
It turns out the existence of such an infinite family of pseudorandom set systems is enough to prove \Cref{thm:Weak-ATV-PAC}. The idea is to consider the set of uniform distributions over the set system and to look at the concept class given by the global labeling restricted to each subset and set to one on the rest of $[N]$. Crucially this has the property that for every distribution, the restricted function corresponding that distribution looks random, but all otther restrictions look like the all ones. This property allows for a small cover and ATV-learnability. On the other hand, we also know that the subsets cannot be distinguished on their intersection, and are promised that landing in such an intersection is reasonably likely. This gives a lower bound against PAC-learning.
\begin{proof}
We argue that \Cref{lemma:set-system} is sufficient to prove the theorem. For every $n \in \mathbb{N}$, let $N$, $M$, and $S_1,\ldots,S_M$ be as in \Cref{lemma:set-system}. Consider the triple $([N],D_{S}, f_S)$ where $D_{S}$ is the set of uniform distributions over each $S_i$, and $f_S$ is contains all functions of the following form:
\[
f_{S_i} = \begin{cases}
f(x) & x \in S_i\\
1 & \text{else}
\end{cases}
\]
We argue that $([N],D_{S}, f_S)$ cannot be PAC-learned up to $1/4$ accuracy in $n$ queries, but is weakly $(4\varepsilon,\delta)$-ATV-learnable and every $D \in D_{S}$ has a $2\varepsilon$-cover of size $2$ with respect to $f_S$. Taking the countable union of these classes maintains the latter two properties while assuring no learner with finite sample complexity can achieve error better than $1/4$.

we first prove every $(D_{S_i},f_S)$ has a small cover. For any fixed distribution $D_{S_i}$, notice that by definition $(D_{S_i}, f_S) $ is $2\varepsilon$-covered by the set:
\[
C_{S_i} = \{ \vec{1}, f_{S_i} \}
\]
since every $f_{S_j}$ for $j \neq i$ has at most a $2\varepsilon$ mass of $0$s. 

We can build a Weak ATV-learner by a similar observation, namely that for any given distribution $D_{S_i}$, every $f_{S_j}$ for $j \neq i$ is nearly the all one's function. Given a sample $S$, the distances assigned by our approximate metric to concepts $f_{S_i}$,$f_{S_j}$ will therefore depend on whether or not $f_{S_i}$ and $f_{S_j}$ are close to the all ones function on $S$. For a given sample $S$, let $C_1(S)$ denote the set of $f_{S_j}$ with empirical density at least $3/4$. We argue that the following mapping $m$ from samples to approximate metrics based on $C_1(S)$ gives the desired learner:
\[
m(S)(f_{S_i},f_{S_j}) = \begin{cases}
  0 & f_{S_i}, f_{S_j} \in C_1(S)\\
1  & \text{else}
\end{cases}
\]
We define the well-approximated set of concepts $G(S,D)$ in the natural manner: For $D=D_{S_i}$, $f_{S_j} \in G(S,D)$ if $j \neq i$ and $f_{S_j} \in C_1(S)$, or $j=i$ and $f_{S_j} \notin C_1(S)$. It is not hard to see that the distances between all pairs in $G(S,D)$ are correctly estimated up to $4\varepsilon$. It is left to show that for every distribution $D_{S_i}$ and concept $f_{S_j}$, $f_{S_j} \in G(S,D_{S_i})$ with  probability at least $1-\delta$, which follows immediately from a Chernoff bound so long as $S=\Omega(\log(1/\delta))$.

Finally, we argue that $([N],D_{S}, f_S)$ cannot be $(1/16,1/8)$-PAC learned in $n$ samples. This is essentially immediate from applying Yao's minimax theorem to the 3rd property. In particular, it is enough to analyze the following basic strategy for the adversary: choose $(D_{S_i},f_{S_i})$ uniformly at random. Given this strategy, let $E$ denote the event that the learner draws a sample $S$ contained in at least two distinct $S_j$ (recall we are promised $E$ occurs with probability at least $1/4$). Fix some sample $S \in E$. We prove that conditioned on $S$, the learner outputs a hypothesis with error greater than $1/16$ with probability at least $1/2$. To see why this is the case, let $\mathcal T$ denote the set of $S_j$ which contain $S$. Notice that the posterior over the adversary's choice of $(D_{S_j},f_{S_j})$ given $S$ is uniform over $S_j \in \mathcal T$. Further these choicecs are 1/16-separated in the following sense: for any $S_j \in \mathcal T$, if the learner outputs $h_S$ s.t. $d_{D_{S_j}}(h_S, f_{S_j}) <1/16$, then properties 2 and 3 imply that that for all $i \neq j$, $d_{D_{S_i}}(h_S, f_{S_i}) > 1/16$. Therefore the learner can only be within $1/16$ error over one of $|\mathcal T| \geq 2$ uniformly random choices. Since E occurs with probability at least $1/4$, we get the desired $(1/16,1/8)$-PAC lower bound.

\end{proof}
\maxh{Note: I have made no attempt at optimizing constants here. They can certainly be improved}


OLD PAC=NON-UNIFORM COVERING (pre-cursor to paper)

\section{PAC-Learning}\label{sec:agnostic-vs-PAC}
In this section we prove the equivalence of realizable and agnostic PAC-learning via a combinatorial object we call a \textbf{probable cover} which may be thought of as a sort of algorithmic variant of a fractional cover. Our algorithm for agnostic learning given a realizable learner $A$ with sample complexity $n(\varepsilon,\delta)$ follows a simple two step procedure:
\begin{enumerate}
    \item Draw an \textit{unlabeled} sample\footnote{One may not have access to an oracle for unlabeled samples, but in this case just draw a labeled sample and ingore the labels.} $S \sim D^{n(\varepsilon/2,\delta/2)}$ and run $A$ on each possible labeling of $S$ under $H$. Call the resulting set of hypotheses $C(S) \subset H$.
    \item Draw $O\left( \frac{\log\left(\Pi_H(n(\varepsilon/2,\delta/2)\right) + \log(1/\delta)}{\varepsilon^2} \right)$ \textit{labeled} samples and output the hypothesis in $C(S)$ with the lowest empirical error.
\end{enumerate}
We will argue below that this process outputs a hypothesis within $\varepsilon$ error of the optimal concept in $H$ with probability at least $1-\delta$. In fact, the above can be shown in only a few lines, but due to connections with other objects we study we will give a longer exposition that introduces a closely related combinatorial object called a probable cover.
\begin{definition}[Probable Cover]
A $(\varepsilon,\delta)$-probable cover of the triple $(X,\mathscr P, H)$ is a function $f: X^n \to P(H)$ such that for any distribution $D \in \mathscr P$ and $h \in H$, the probability over samples $S \sim D^n$ that $h$ is $\varepsilon$-close to some hypothesis in $f(S)$ with probability at least $1-\delta$:
\[
\forall D \in \mathscr{P}, h \in H: \Pr_{S \sim D^n}\left[\exists h' \in f(S) : d_D(h',h) \leq \varepsilon \right] \geq 1-\delta.
\]
We call $n$, which should be thought of as the computational cost to ``sampling'' the approximate cover, the \textbf{cost} of $f$, and denote it in the following by $c(f)$. Moreover, the \textbf{size} of $f$, denoted by $|f|$, is given by the largest cardinality of its output. We call a probable cover \textbf{bounded} if has finite size. 
\end{definition}
\maxh{We should think about a cleaner way to define this and/or connections with classical objects}
It is not hard to see that PAC-learning is exactly equivalent to the existence of bounded probable covers.
\begin{proposition}\label{prop:PAC-cover}
$(X,\mathscr P, H)$ is PAC-learnable in the realizable setting if and only if $\forall \varepsilon,\delta > 0$ it has a bounded $(\varepsilon,\delta)$-probable cover. Moreover, the sample complexity of PAC-learning $(X,\mathscr P, H)$ is closely related to the minimal size and cost of a probable cover in the following sense. For any probable cover $f$, we have:
\begin{align*}
   n(\varepsilon,\delta) \leq O\left(c(f) + \frac{\log(|f|)+\log(1/\delta)}{\varepsilon}\right)
\end{align*}
Similarly, a PAC-learner using $n(\varepsilon,\delta)$ samples implies the existence of an $(\varepsilon,\delta)$-probable cover $f$ satisfying:
\begin{align*}
    c(f) &\leq n(\varepsilon,\delta)\\
    |f| &\leq \Pi_H(n(\varepsilon,\delta))
\end{align*}
where $\Pi_H(m)$ is the growth function and counts the maximum number of labelings given by H across sets of size $m$.
\end{proposition}
\begin{proof}
We start with the forward direction. Assume the existence of a $(\varepsilon/2,\delta/2)$-probable cover $f$. Draw a sample $S \sim D^n$ to receive $f(S)$. Notice that for any $h \in H$, the probability that $f(S)$ $\varepsilon/2$-covers $h$ is at least $1-\delta/2$. Recall that by assumption, $|f(S)|$ is finite. Then by standard arguments, drawing $O\left( \frac{\log(|f(S)|)+\log(1/\delta)}{\varepsilon}\right)$ samples and choosing $h' \in f(S)$ with the lowest empirical error gives the desired PAC-learner.

For the backward direction, assume conversely that we have access to a $(\varepsilon,\delta)$-PAC learner. For each sample $S \in X^{n(\varepsilon,\delta)}$, let $f(S)$ be the set of outputs obtained by running the PAC-learner on all $\Pi_H(S)$ realizable labelings. It is immediate from the definition of PAC-learnability that $f$ is a $(\varepsilon,\delta)$-probable cover of size $\Pi_H(n(\varepsilon,\delta))$. Namely, for any $D \in \mathscr{P}$ and $h \in H$, the output of a PAC-learner on $S,h(S) \sim D^{n(\varepsilon,\delta)}$ (which is by definition included in $f(S)$) is $\varepsilon$-close to $h$ with probability at least $1-\delta$. The size bound follows immediately from the definition of the growth function.
\end{proof}
By almost exactly the same argument, we can prove that a probable cover gives an \textit{agnostic} learning algorithm. Since a PAC-learner gives a probable cover (and is trivially weaker than agnostic learning), this implies the desired equivalence.
\begin{corollary}\label{cor:real-to-agn}
$(X,\mathscr{P},H)$ is PAC-learnable in the realizable setting if and only if it is PAC-learnable in the agnostic setting. Moreover, the sample complexity of agnostic learning is at most:
\[
n_A(\varepsilon,\delta)  \leq O\left( \frac{\log\left(\Pi_H(n(\varepsilon/2,\delta/2)\right) + \log(1/\delta)}{\varepsilon^2} \right) \leq O\left( \frac{n(\varepsilon/2,\delta/2) + \log(1/\delta)}{\varepsilon^2} \right)
\]
\end{corollary}
\begin{proof}
The forward direction is trivial. The backward direction is essentially the same as in \Cref{prop:PAC-cover}. In particular we can use the PAC-learner to generate a probable cover with cost $c(f)=n(\varepsilon/2,\delta/2)$ and size $\Pi_H(n(\varepsilon/2,\delta/2))$. Draw a sample $S \sim D^{c(f)}$. For any $h$, $f(S)$ $\varepsilon/2$-covers $h$ with probability
at least $1-\delta/2$. Standard arguments give that the loss of all concepts in $f(S)$ may be jointly estimated up to $\varepsilon/2$-accuracy in $O\left( \frac{\log\left(\Pi_H(n(\varepsilon/2,\delta/2)\right) + \log(1/\delta)}{\varepsilon^2} \right)$, so outputting the concept with the lowest empirical error gives the desired agnostic learner.
\end{proof}



% let $C(S)\subset H$ be the set of hypothesis consistent with $S$ i.e. $f_i \in C(S)$ if and only if $S$ is consistent with distribution $D_i$.  Then, we define our metric $d_S$ as
\iffalse
\[
d_S(f_j, f_k) =\begin{cases}
1/2 & f_j \in C(S) \land f_k \notin C(S) ~\text{or}~ f_j \notin C(S) \land f_k \in C(S)\\
(\epsilon_j/2) (1- \epsilon_k/2) +  (\epsilon_k/2) (1- \epsilon_j/2) & f_j \notin C(S) \land f_k \notin C(S)\\
0 & f_j \in C(S) \land f_k\in C(S)
\end{cases}
\]
of size $O(\frac{1}{\epsilon_i}\log(1/\delta))$, \begin{enumerate}
    \item $f_i \in C(S)$ with probability 1.
    \item $f_j \notin C(S)$ for any $j \neq i$ with probability $1-\delta$.
\end{enumerate}
\fi
% \[
% d_S(f_j, f_k) =
% (\epsilon_j/2) (1- \epsilon_k/2) +  (\epsilon_k/2) (1- \epsilon_j/2) 
% \]
% Its clear from above that for any $S\sim D_i$, $d_S$ is correct for all hypothesis $f_j, f_k$ for $j, k \neq i$. In fact, the metric is correct on all hypothesis except $f_i$ which proves 1).



UNIFORM ESTIMATION:

In this section, we refute a strong variant of the uniform estimation hypothesis, providing an example of a class which is PAC-learnable but not strongly ATV-learnable.


\begin{theorem}\label{thm:TV-not-necessary}
 There exists a class $(\mathscr{D},X,H)$ which is PAC-learnable in $\tilde{O}(\frac{\log(1/\delta)}{\varepsilon})$ samples but is not strongly $(1/3,1/3)$-ATV learnable.
\end{theorem}
Note that this immediately disproves the weaker uniform estimation hypothesis by \Cref{thm:TV-Estimation}.
\begin{corollary}
There exists a class $(\mathscr{D},X,H)$ which is PAC-learnable in $\tilde{O}(\frac{\log(1/\delta)}{\varepsilon})$ samples but has no $(1/3,1/3)$-uniform estimator.
\end{corollary}

We'll start by overviewing the construction, which is in essence based on learning dictator functions on the noisy hypercube. 
%In particular, we will build an infinite sequence of classes $\{H^\varepsilon_n\}$ which are learnable up to $\varepsilon$ error in $O_\delta(1)$ samples, but require a growing number of samples to uniformly estimate. \Cref{thm:TV-not-necessary} will then follow from stringing together an infinite sequence of these classes.
Namely, consider the class $\mathcal{H}_n^\varepsilon =(\mathscr{D}_n^\varepsilon, \{0,1\}^n, H_n)$, where $H_n \coloneqq \{ \mathbf{1}_x : x \in [n]\}$ is the set of all dictators on the cube
\[
\mathbf{1}_x(T) = \begin{cases}
1 & \text{if } x \in T\\
0 & \text{else}
\end{cases}
\]
and $\mathscr{D}_n^\varepsilon \coloneqq \{ D^\varepsilon_S : S \subset [n]\}$ is the set of $\varepsilon$-noisy binary strings (in the sense that $D^\varepsilon_S$ is given by flipping each bit in $S \in \{0,1\}^n$ independently with probability $\varepsilon$). We first claim that any fixed such class is PAC-learnable up to error $\varepsilon$, but has no uniform estimator that is independent of the class size $n$.
\begin{proposition}\label{prop:finite-lower}
 For any $\delta>0$ and $1/6 > \varepsilon > 0$, $(\mathscr{D}_n^\varepsilon, \{0,1\}^n, H_n)$ is learnable up to $\varepsilon$ error with probability at least $1-\delta$ in $O(\log(1/\delta))$ samples, but any $(1/3,1/3)$-ATV learner must use at least $\Omega(\frac{\log(n)}{\log(1/\varepsilon)})$ samples.
\end{proposition}
\begin{proof}
We first argue learnability, which is the easier of the two by far. Observe that by construction, no matter the distribution and hypothesis chosen by the adversary our class is `almost constant:'
\[
\forall D^\varepsilon_S \in \mathscr{D}_n^\varepsilon, h_x \in H, \exists z \in \{0,1\}: Pr_{T \sim D^\varepsilon_S}[h_x(T) = z] = 1-\varepsilon.
\]
This is immediate from the fact that every coordinate in $D_S$ is equal to its value in $S$ with probability exactly $1-\varepsilon$. There is then an obvious learning strategy: after $O(\log(1/\delta))$ samples, output the majority value (as a constant function).\footnote{We note this can be made `proper' simply by adding the all $0$'s and all $1$'s function to the class. This only makes uniform estimation harder, so it does not effect the lower bound.} For any small enough $\varepsilon$ (say at most $1/4$), this outputs the measure $1-\varepsilon$ element with probability at least $1-\delta$, which gives the desired result.

Showing any uniform estimator requires $\Omega(\frac{\log(n)}{\log(1/\varepsilon)})$ samples is slightly more involved, but the idea is simple: when $n$ is large (with respect to $\varepsilon$ and the sample size of the estimator), there is likely to be at least one coordinate whose majority value is flipped by the noise. Since our function class is made up of dictators, building a uniform estimator would require detecting where such flips occur, but this is an impossible task since the values on other coordinates are independent and provide no relevant information. More formally, we will break the proof into two parts. First, we'll show that we can reduce to analyzing the natural `majority' strategy. Second, we'll show this strategy fails with high probability.

Before this, however, it will be convenient to slightly rephrase the problem. Notice that for $\varepsilon < 1/4$, a $(1/3,1/3)$-uniform estimator on $t$ samples implies the existence of an algorithm $\mathcal{A}$ with the following guarantees: given $t$ samples from $D^\varepsilon_S$, $\mathcal{A}$ outputs $S$ with probability at least $1/3$. This follows from the fact that for any fixed $D^\varepsilon_S$ and $h_i$, the error of $h_j$ is less than $2\varepsilon$ if $S(i)=S(j)$, and more than $1-2\varepsilon$ if $S(i)\neq S(j)$. As long as $2\varepsilon < 1/3$, a $(1/3,1/3)$-uniform estimator can distinguish between these cases unless it fails altogether. 

Thus it is enough to show that any algorithm which correctly outputs the underlying string $S$ with at least $1/3$ probability uses many samples. By Yao's minimax principle, it is enough to show the adversary has a strategy such that any deterministic algorithm to this end fails with high probability. The adversary will simply choose a uniformly random distribution from $\mathscr{D}^\varepsilon_n$. As discussed, we first argue that the best strategy for outputting $S$ is to output majority for each coordinate. To see this, we think of the choice of $S$ and sample $T$ as a jointly distributed variable, and marginalize over the samples and consider the conditional failure rate of the algorithm:
\begin{align*}
    \Pr_{S \sim \{0,1\}^n, T \sim D_S^\varepsilon}[A(T) \neq S] = \sum\limits Pr[T_0]\Pr[A(T) \neq S | T =T_0]
\end{align*}
Notice that the conditional probability $\Pr[A(T) \neq S | T =T_0]$ is just one minus the posterior probability of $A(T_0)$, so the error is minimized by choosing the maximum posterior element in the posterior. Since our prior distribution over $S$ is uniform, the posterior is maximized by choosing the majority element in each coordinate.

Finally, it is left to argue that the majority rule fails with high probability. This follows from the fact that unless our sample size is large, there will almost always be some coordinate which is flipped by noise in every sample. In particular, recall that each coordinate is flipped independently with probability $\varepsilon$. The probability that there exists at least one coordinate that is flipped in each of $t$ samples is then $1-(1-\varepsilon^t)^n$. Taking $t \leq \frac{c\log(n)}{\log(1/\varepsilon)}$ for some small enough absolute constant $c$ gives that this probability is at least $2/3$ which gives the desired lower bound.

\end{proof}
Finally we argue that taking the disjoint union of infinitely many such instances gives the full result.
\begin{proof}[Proof of \Cref{thm:TV-not-necessary}]
For any increasing super-polynomial function $m(\varepsilon)$, consider the disjoint union of classes $\bigcup_{n \in \mathbb{N}}\mathcal{H}_n^{m^{-1}(n)}$. We first prove this class is PAC-learnable. Given any $\varepsilon,\delta > 0$, we consider two cases. In the first case, the adversary selects a distribution/hypothesis pair indexed by $n$ such that $m^{-1}(n) \leq \varepsilon$. In this case, PAC-learnability follows exactly the same argument as in \Cref{prop:finite-lower}. Otherwise, the adversary selects $n \leq m(\varepsilon)$. In this case there are only $m(\varepsilon)$ hypotheses, so simple empirical risk minimzation outputs a good hypothesis in $O(\frac{\log(m(\varepsilon))+\log(1/\delta)}{\varepsilon})$ samples. Finally note these cases can be distinguished by the learner in one sample, since each instance space is `marked' by its corresponding index (value of $n$).

On the other hand, it is easy to see there cannot be any bounded $(1/3,1/3)$-uniform estimator for this class. For any fixed sample size $t$, the adversary can always choose $n$ such that $t \ll \log(n)/\log(1/m^{-1}(n))$ (since $m$ is super-polynomial). \Cref{prop:finite-lower} implies $\mathcal{H}_n^{m^{-1}(n)}$ has no $(1/3,1/3)$-uniform estimator, which completes the proof.

\end{proof}

% \subsection{Uniform Estimation in the Universal Model}
% One common complaint about the standard PAC setting is that the adversary gets to `see' the number of samples (i.e. worst case examples are given for a fixed sample complexity). On the other hand, in practice the classifier and underlying distribution are often thought of as fixed, and one analyzes the `learning curve' which plots the generalization error as samples tend to infinity. Indeed, this dependence on number of samples is crucial in our refutation of the uniform estimation hypothesis. If the adversary's choice is fixed before the number of samples, then it is indeed possible to build a `bounded' uniform estimator for the class (where the number of samples depends on the adversaries choice of $n$). This raises a natural question: to what extent does uniform estimation hold in this `universal' model? We show a strong negative result in this direction.

% \begin{theorem}
% There exists a class $(\mathscr{D},X,H)$ that is PAC-learnable in $1$ sample, but has no (measurable) uniform estimator in the universal model.
% \end{theorem}



% In this work, we revisit this model from a new angle: \textit{unsupervised} learning.
% Unsupervised learning is a mainstay of modern ML, from classical methods such as clustering \cite{lloyd1982least,macqueen1967classification} and dimensionality reduction \cite{pearson1901liii,fodor2002survey}, to more involved applications in modern methods such as deep learning \cite{ouali2020overview}. The paradigm has also proved powerful in statistical learning theory, where multi-stage learners that infer information from unlabeled data before applying traditional supervised approaches underlie state-of-the-art algorithms across a wide variety of settings \cite{balcan2010discriminative, beimel2013private,alon2019limits,hopkins2020point,diakonikolas2022strongly}.
% We consider a common paradigm that has seen extensive use
% In the 30 years since these works, our understanding of the foundational distribution-family model has remained largely stagnant, while progress in machine learning practice and related theoretical models capturing distributional or data-dependent assumptions have flourished (e.g.\ margin-based algorithms \cite{freund1998large}, learning halfspaces \cite{blum1998polynomial}, semi-supervised learning \cite{balcan2010discriminative}, active learning \cite{balcan2007margin}).
% A crucial component of such works, also seen frequently in machine learning practice, is to start by learning relevant features of the underlying marginal distribution over raw data, then train a classifier based on this information over a fresh set of labeled samples.
% \footnote{In fact, recently such methods have even proved useful in traditional PAC learning, leading for instance to strongly polynomial time algorithms for halfspaces \cite{diakonikolas2022strongly} (albeit improperly).} 

% The distribution family model comes with an inherent unsupervised analog: given a triple $(\mathscr{P},X,H)$, is it possible to `learn' the adversary's choice of $D \in \mathscr{P}$ with respect to some natural $H$-dependent metric? Given the close interplay between supervised and unsupervised methods in modern ML, one might hope to show these problems are in fact, equivalent. After all, solving the unsupervised problem seems like it should be sufficient, since one can then just learn $(D,H)$ directly,\footnote{It is trivially necessary of course that each pair $(D,H)$ is learnable, this is captured by assuming the class has UBME which we have ignored here for simplicity and discuss later on.} while inferring some information about $D$ is also clearly necessary to output a good hypothesis. In fact, the truth is more subtle. 

% While this fails to give a full characterization, it represents essentially the first non-trivial step beyond the failure of uniform convergence and covering numbers in understanding the structure of learnable classes under arbitrary distributional assumptions.
% \shachar{you use STV, WTV here, but the full name Strong TV, Weak TV in Theorem 1.1. I suggest to use consistent naming.}

% The proof of \Cref{intro:thm-char} relies on an independently interesting connection between TV-learning and a relaxed variant of uniform convergence called \textit{uniform estimation}.
% % The familiar reader may notice the flavor of TV-learnability is closely connected to the idea of uniform convergence, that we wish to estimate some features of (most of) $H$ with respect to the underlying distribution uniformly. Indeed this can be made formal through the idea of 
%  While uniform convergence is the promise that the \textit{empirical error} of every $h \in H$ approaches its true error uniformly, uniform estimation relaxes this requirement to the existence of \textit{any} good estimator for error in $H$. While Benedek and Itai showed uniform convergence is not necessary for learnability under fixed distributions, uniform estimation actually is necessary in both the fixed and distribution-free settings, so it is natural to conjecture this holds in general. We refute this conjecture by showing uniform estimation is equivalent to (Exact) TV-learning. \shachar{this is another new definition, we need to define all these more precisely}
% \begin{corollary}[Refuting the Uniform Estimation Hypothesis]\label{intro:estimation}
% There exists a class $(\mathscr{P},X,H)$ which is PAC-learnable but has no uniform estimator.
% \end{corollary}
% In fact, we prove a variant of this result even for a weak form of uniform estimation that just promises a large known set of hypotheses are well-estimated in each round (akin to STV-learning).

% \begin{proposition}
% If $(D,H)$ is learnable $\forall D \in \mathscr{P}$:
% \[
% \text{TV-learnability $\iff$ Uniform estimation}
% \]
% \end{proposition}
% The PAC-TV Sandwich Theorem is also inherently connected to classical paradigms in learning such as covering numbers and uniform convergence. As a result, \Cref{intro:main-thm} can be used to refute several variants of classical conjectures or `paradigms' that typically characterize worst-case models of supervised learning. First, we prove that (under bounded UBME) basic `TV-learnability' is exactly equivalent to the existence of a good \textit{uniform estimator}, a function which intakes labeled samples and outputs a a good estimate for the error of every $h \in H$. Since TV-learning is contained in Strong ATV-learning, this refutes a natural weakening of the UCH called the `\textit{uniform estimation hypothesis}':
% \begin{corollary}[Refuting the Uniform Estimation Hypothesis]
% There exists a class $(\mathscr{P},X,H)$ which is PAC-learnable but has no uniform estimator.
% \end{corollary}
% Second, we prove that UBME and TV-learnability is also equivalent to the ability to construct a cover for $H$ from a bounded number of samples along with its corresponding covering map. As such, \Cref{intro:main-thm} refutes natural covering-based characterizations of learning as well.
% \begin{corollary}[Refuting the Uniform Covering Hypothesis]
% There exists a class $(\mathscr{P},X,H)$ which is PAC-learnable, but has no covering algorithm.
% \end{corollary}


% In other words, $(\mathscr P, X, H)$ is TV-learnable if it is possible to estimate the measure of every event in $H \Delta H$ from a bounded number of unlabeled samples. TV-learning is a very strong notion of learnability that falls into what might be considered the \textit{uniform convergence paradigm} (where everything is simultaneously well-estimated). Indeed, we will later formalize this connection with a generalization of this paradigm called \textit{uniform estimation}. 
% This leads to the following conjecture we call the ``uniform estimation hypothesis:''
% \begin{conjecture}\label{conj:TV}
% A class $(\mathscr{P},X,H)$ is PAC-learnable iff it has a uniform estimator (equivalently is TV-learnable $+$ UBME).
% \end{conjecture}

% On the other hand, it is easy to see that TV-learning and uniform estimation may be unnecessarily strong for learning in a couple of ways. First, it is worth noting that we do not really need access to a distribution estimating the true marginal. It is enough to have a metric that approximates the distance between any two hypotheses $h,h' \in H$. Second, it is not strictly necessary to uniformly estimate \textit{all} the hypotheses---we will see learning is still possible as long as a significant (and known) portion of hypotheses have good distance estimates. Toward this end, we call $(\mathscr P, X, H)$ Strongly ATV-learnable if it is possible to estimate the standard distance metric $d_D(h,h') = D(h \Delta h')$ from a bounded number of samples drawn from $D \in \mathscr P$ such that the well-approximated distances are \textbf{known to the learner}. More formally,


APX UE:

% In fact, we will consider an even weaker form that only requires uniformity over `most' hypotheses (akin to the requirement of STV-learning).
% \begin{definition}[Approximate Uniform Estimation]
% We say a class $(\mathscr{P},X,H)$ has the approximate uniform estimation property if for all $\varepsilon,\delta >0$ there exists a function $n(\varepsilon,\delta)$, an estimator $f: S \times H \to \mathbb{R}_+$, and a distinguisher $G: S \to P(H)$ such that 

% \begin{enumerate}
%     \item The error of every hypothesis in $G(S)$ is simultaneously well-estimated by $f$ with high probability:
% \[
% \forall D \in \mathscr{P}, h \in H:
% \Pr_{S \sim D^n}[\exists h' \in G(S): |f((S,h(S)),h') - d_D(h',h)| > \varepsilon] \leq \delta.
% \]
% \item Every $h \in H$ appears in $G(S)$ with high probability:
% \[
% \forall D \in \mathscr{P}, h \in H:
% \Pr_{S \sim D^n}[h \in G(S)] \geq 1- \delta.
% \]
% \end{enumerate}
% \end{definition}




% Note that given $(C^\varepsilon,c)$, it is easy to recover both uniform estimation and TV-learnability. The former is immediate from Chernoff and union bounds by outputting the empirical error of $c(h)$ on sufficiently many samples, and the latter follows similarly from computing the (empirical) pairwise distance of elements in the cover over sufficiently many samples and letting $d(h,h')=\hat{d_S}(c(h),c(h'))$.

% It is left to prove that uniform estimation and TV-learnability imply the ability to build such a pair $(C^\varepsilon,c)$. We start with the former. Since $(\mathscr{P},X,H)$ is TV-learnable, we can output a distribution $D' \in \mathscr{P}$ such that $TV_{H \Delta H}(D',D) \leq \varepsilon/2$. Since $(\mathscr{P},X,H)$ has UBME, the distribution $D'$ has a bounded $\varepsilon/2$-cover $C^{\varepsilon/2}_{D'}$. Since $D'$ is known, the corresponding covering map $c_{D'}$ is known as well. Finally, since $TV_{H \Delta H}(D',D) \leq \varepsilon/2$, $(C^{\varepsilon/2}_{D'},c_{D'})$ gives the desired $\varepsilon$-covering + covering-map pair for $D$.

% On the other hand, if we have a uniform estimator note that the class is learnable simply by outputting the hypothesis with minimum measured error. It is proved in \cite{hopkins2021realizable} that it is always possible to generate a uniformly bounded $\varepsilon/4$-cover $C^\varepsilon$ for any learnable class in a uniformly bounded number of samples. Run the uniform estimator for every hypothesis in the cover $C^\varepsilon$, and build a covering map simply by mapping each $h \in H$ to some center it is within $\varepsilon/2$ of.
% Modifying the argument to the approximate setting follows similarly, where the uniform cover is built only for a known set $G(S) \subset H$ s.t. any $h \in G(S)$ with high probability.

% Thus the only difference between the strong and weak models are whether the learner knows the set of well-estimated elements. We prove that any learnable class 

% Unfortunately, in the distribution-family case, Strong TV learning does indeed end up 

% In other words, a class is strongly TV learnable if it is possible to estimate $H \Delta H$ on most elements

% We show that the distribution family PAC-model is strictly sandwiched between two natural notions of unsupervised learning with respect to this metric:
% % The answer to this question, it turns out, is subtle, and depends on how you quantify `learnability' with respect to class-conditional TV-distance. We study two such notions
% \textit{`Weak' TV-learning} (WTV), in which the learner has a good estimate for the measure of most events in $H \Delta H$, and \textit{`Strong' TV-learning} (STV) which promises the same with the additional guarantee that the learner \textit{knows} the set of well-estimated events.
% \shachar{since STV,WTV definitions are central to the paper, and are new, I suggest to describe them more formally here, or at the very least give the ref where they are formally defined}

% \footnote{Note the `Strong' setting a weakening of learning $D$ in $TV_{H \Delta H}$ distance, where one is promised to have good estimates on the entirety of $H \Delta H$.} 
% While on the surface it is not even clear these definitions differ, we show PAC-learning is in fact strictly sandwiched between them.
% We study a refinement of this question based upon two notions of approximate TV-learnability. At a high level, the first of these variants, called (Weak) ATV-learnability, promises the ability to map an unlabeled sample S to an approximate distance metric $d_{S}: H \times H \to \mathbb{R}$ such that the true distance between every pair $(h,h')$ is well-estimated with high probability.
% % \[
% % \forall h,h' \in H: \Pr_S[d_S(h,h') \approxeq d_D(h,h')] \geq 1-\delta
% % \]
% The second, called (Strong) ATV-learnability, promises the same, but crucially \textit{reveals} the set of well-estimated pairs as well. We prove that PAC-learning lies strictly sandwiched between Weak and Strong ATV-learning:

% model fails to capture many properties of learnability observed in practice. 
% Deep neural nets and other modern architectures, for instance, seem to learn much faster than classical tools like uniform convergence would predict, and frequently rely on more complex learning rules than simply minimizing empirical error. 
% One commonly cited reason for this difference is that real-world data sets aren't truly adversarial: the highly structured, combinatorial marginal distributions used for classical lower bounds simply don't appear in practice. This simple observation has driven decades of progress in modern learning theory, from the development of efficient algorithms over fixed marginal distributions \cite{benedek1991learnability} to data-dependent scenarios like learning with margin \cite{freund1998large} or techniques such as semi-supervised learning \cite{balcan2010discriminative} which take advantage of distributional information. Yet, at a statistical level, most foundational questions beyond the distribution-free case remain wide open:

% At a high level, the idea is to observe that when $n$ is large (with respect to $\rho$ and the sample size of the estimator), there is likely to be at least one coordinate whose majority value is flipped by the noise. Since our function class is made up of dictators, building an STV-learner requires detecting where such flips occur, but this is an impossible task since the values on other coordinates are independent and provide no relevant information.

% To formalize this, it will be convenient to slightly rephrase the problem. Notice that for $\rho < 1/6$, a $(1/3,1/6)$-STV-learner on $t$ samples implies the existence of an algorithm $\mathcal{A}$ with the following guarantees: given $t$ samples from $D^\rho_W$, with probability at least $1/6$ $\mathcal{A}$ outputs a string $x \in \{0,1,\bot\}^n$ such that\footnote{Algorithms with this type of guarantee are well-studied in the learning literature under a variety of names such as ``Reliable and Probably Useful'' \cite{rivest1988learning},  ``Confident'' \cite{kane2017active}, or ``Knows What It Knows'' \cite{li2001improved}.}
% \begin{enumerate}
%     \item $x$ is `$\bot$' on at most $n/2$ coordinates
%     \item $x$ agrees with $W$ otherwise. 
% \end{enumerate}
% This can be seen via the following process. Draw $t$ samples from $D^\rho_W$, and run the STV-learner to get $\tilde{d}_T$ and $G_T$. The idea is to observe that we can use $\tilde{d}_T$ to determine the relative values \shachar{???} of all elements in $G_T$. Then as long as we can label one such element correctly, we can label all elements in $G_T$ correctly and output `$\bot$' on the rest.


% More formally, let $W_i$ denote the value in the $i$th coordinate of $W$, and observe that the true distance between the indicators of $i,j$ is $d(\mathbf{1}_i,\mathbf{1}_j) \leq 2\rho < 1/3$ whenever $W_i = W_j$, but at least $d(h_1,h_i) \geq 1-2\rho > 2/3$ when $W_i \neq W_j$. Since our approximate distance metric is $1/3$-accurate on $G_T$, this means we can determine $|W_i-W_j|$ for every $\mathbf{1}_i,\mathbf{1}_j \in G_T$. We can then use the following process to output a string $\widehat{W}$: if $\mathbf{1}_1 \in G_T$, define $\widehat{W}_1$ to be the majority value of coordinate $1$ across our sample, and assign all other coordinates in $G_T$ by their relative value with respect to $\widehat{W}_1$ (output `$\bot$' in all other settings). The majority value and approximate metric are each correct with probability at least $5/6$. Moreover, since the probability any $\mathbf{1}_x \in G_T$ is at least $5/6$, Markov's inequality promises $|G_T| \geq n/2$ with probability at least $2/3$. Finally, since $\mathbf{1}_1 \in G_T$ with probability at least $5/6$, union bounding over all events implies that with probability at least $1/6$, the algorithm correctly outputs $\widehat{W}_\ell=W_\ell$ for all (at least) $\frac{n}{2}$ coordinates where $\mathbb{1}_\ell \in G_T$ and answers $`\bot'$ on any remaining coordinates as desired.

